FrUITeR: A Framework for Evaluating UI Test Reuse

UI testing is tedious and time-consuming due to the manual effort required. Recent research has explored opportunities for reusing existing UI tests from an app to automatically generate new tests for other apps. However, the evaluation of such techniques currently remains manual, unscalable, and unreproducible, which can waste effort and impede progress in this emerging area. We introduce FrUITeR, a framework that automatically evaluates UI test reuse in a reproducible way. We apply FrUITeR to existing test-reuse techniques on a uniform benchmark we established, resulting in 11,917 test reuse cases from 20 apps. We report several key findings aimed at improving UI test reuse that are missed by existing work.

==> related.tex <==
\section{Related Work}
\label{sec:related}

==> rq.tex <==
\section{Research Questions}
\label{sec:rq}

\begin{comment}
	In this paper, we specifically focus on 
(1) the granularity of UI tests to be reused (replacing \textbf{Test Processor}); 
(2) the reusability of different benchmark apps (replacing \textbf{Test Selector}); 
and (3) the suitability of different GUI match algorithms (replacing \textbf{GUI Matcher}). 
Other RQs can be explored with \framework~ in the same manner by replacing other components, such as replacing \textbf{Test Generator}  to explore the reusability of the UI tests generated by different test generation techniques.

\subsection{Granularity of Tests to be Reused}
\yixue{We should probably rename "test to be reused", e.g., donor tests or something. Will think about it when writing framework design.}

Determining the granularity of the UI tests is an essential step in test reuse as it has direct impact on the reusability and usefulness of the tests to be used. 
For instance, a complex test with long event sequence is likely to be app-specific, thus is hard to be reused by other apps. 
On the other hand, a test that is too simple (e.g., containing only one GUI event) can easily be reused, but will not yield meaningful UI tests. The authors of
\appflow~ \cite{hu2018appflow} suggest that tests should be kept simple as a best practice based on their experience in writing reusable UI tests, but they do not provide concrete guidelines on how to construct a \emph{simple} test. 

Thus, we quantify the \emph{granularity} of UI tests based on the event sequence length in a certain test (i.e., test length), aiming to explore the suitable granularity that can yield reusable UI tests with the following research question.

\begin{itemize}
\item \textbf{RQ$_1$} -- What is the suitable test length to yield tests that can be successfully reused? 
\end{itemize}

\yixue{We can explore other ways to study tests with different granularity if time/space allows, e.g., divide test cases based on each assertion or based on each UI change, etc. We can run pilot study to see which hypothesis is more interesting/promising and decide later.}

\subsection{Reusability of Tests from Different Apps}

With the tests at proper granularity studied by \textbf{RQ$_1$}, the immediate next question is to study which donor apps are suitable to reuse such tests from, given a specific AUT of developer's interest \yixue{what donor app and AUT stand for will be explained in "framework design" section, which will be before RQ section}. To that end, we ask the following research questions to answer how reusable the tests are from different donor apps given certain characteristics of the AUT, in order to guide developers to select donor apps to apply test reuse techniques.

\begin{itemize}
\item \textbf{RQ$_2$} -- How reusable are the tests from the apps in the same app category?
\item \textbf{RQ$_3$} -- How reusable are the tests from the apps developed by the same developers?
\end{itemize}

\yixue{"how reusable" means the success rate of transferring tests. If time/space allows, we can explore different heuristics to find suitable apps to reuse tests from, e.g., apps with similar Activity transition graphs, apps with similar UI layouts, apps with a large number of code clones, etc...}

\subsection{Suitability of GUI Matcher}

\framework's \textbf{GUI Matcher} is one of the core components that are shared among different test reuse techniques as it defines the core algorithm to reuse UI tests based on the UI similarity between the donor app and the AUT. 
However, \textbf{GUI Matcher} in existing techniques use different metrics and algorithms to calculate UI similarity among different benchmark apps, thus what metrics and algorithms are more suitable for GUI match is unclear. 
For instance, \guitest~ considers the action and text associated with the GUI element to calculate similarity score based on \emph{Wu and Palmer} measure \cite{wu1994verbs}, while \appflow~ \cite{hu2018appflow} leverages machine learning techniques and explore various features and learning algorithms.

Inspired by \appflow~ \cite{hu2018appflow}, we aim to explore the suitability of different \textbf{GUI Matchers} with the following research questions.		
\end{comment}

